Neural Scene Graphs for Dynamic Scenes

Recent implicit neural rendering methods have demonstrated that it is possible to learn accurate view synthesis for complex scenes by predicting their volumetric density and color supervised solely by a set of RGB images. However, existing methods are restricted to learning efficient representations of static scenes that encode all scene objects into a single neural network, and lack the ability to represent dynamic scenes and decompositions into individual scene objects. In this work, we present the first neural rendering method that decomposes dynamic scenes into scene graphs. We propose a learned scene graph representation, which encodes object transformation and radiance, to efficiently render novel arrangements and views of the scene. To this end, we learn implicitly encoded scenes, combined with a jointly learned latent representation to describe objects with a single implicit function. We assess the proposed method on synthetic and real automotive data, validating that our approach learns dynamic scenes -- only by observing a video of this scene -- and allows for rendering novel photo-realistic views of novel scene compositions with unseen sets of objects at unseen poses.

==> background.tex <==
\section{Background}\label{ch:background}
Before presenting the proposed method for dynamic scenes, we review Neural Radiance Fields
(NeRF) by Mildenhall et al.~\cite{mildenhall2020nerf} as a successful approach for learning
static scene representations from a collection of images, under the assumption of
consistency between view points. In NeRF, scenes are modeled by a continuous, volumetric scene function
$F_{\theta}:(\boldsymbol{x}, \boldsymbol{d}) \rightarrow (\boldsymbol{c}, \sigma)$, approximated
using a multilayer perceptron (MLP), which encodes the scene in its weights.
Inputs to the volumetric scene approximation function are a position in Euclidean space $\boldsymbol{x} = (x, y, z)$ and a unit vector viewing direction
$\boldsymbol{d}=(d_x, d_y, d_z)$ which map to a volumetric density $\sigma$ and a RGB
color $\boldsymbol{c}=(r,g,b)$. The architecture for the MLP can be decomposed into two sets of
linear layers, the first of which is described in Eq.
\eqref{eq:nerf_mlp_1} and takes the position $\boldsymbol{x}$ and maps it to a density,
$\sigma$. The model's second set of linear layers maps the viewing direction $\boldsymbol{d}$
concatenated with the output feature vector of the first component to a color $\boldsymbol{c}$, as
in Eq.~\eqref{eq:nerf_mlp_2}. This MLP's architecture ensures consistency of the encoded scene
across camera views by having the volumetric density depend only on the 3D position, and varying
color with viewing position.
\begin{align}
\label{eq:nerf_mlp_1}
[\boldsymbol{y}(t), \sigma(t)] &= F_{\theta_1}(\gamma_{\boldsymbol{x}}(\boldsymbol{r}(t))) \\
\label{eq:nerf_mlp_2}
\boldsymbol{c}(t, \boldsymbol{d}) &= F_{\theta_2}(\gamma_{\boldsymbol{d}}(\boldsymbol{d}), \boldsymbol{y}(t))
\end{align}

Experiments \cite{mildenhall2020nerf, tancik2020fourier} have shown that learning functions
which map from low dimensional problem spaces to high-frequency features can be improved
significantly by adding Fourier feature mappings. Therefore, it is beneficial to apply this
feature encoding to all low dimensional inputs like 3D positions and directions.

The synthesized views are rendered by tracing rays $\boldsymbol{r}(t)$ of a pinhole camera model
through the described volumetric scene representation. With NeRF, the pixel value is
approximated using a volumetric integration between a near and far distance along each ray $t_n$ and $t_f$,
using the equation $\boldsymbol{r}(t) = \boldsymbol{o}+t\boldsymbol{d}$ to sample at equal
distances along the ray. The following integral is then used to compute transmitted color from
the scene along each ray

\begin{equation}
\label{eqn:rendering_integral}
\boldsymbol{C}(\boldsymbol{r}) = \int_{t_{n}}^{t_{f}} T(t)\sigma(\boldsymbol{r}(t))\boldsymbol{c}(\boldsymbol{r}(t), \boldsymbol{d})dt,
\end{equation}
\begin{equation}
\label{eqn:accumulate_transmittance_integral}
\mathrm{where \:} T(t)=\mathrm{exp}(- \int_{t_{n}}^{t} \sigma(\boldsymbol{r}(s))ds,
\end{equation}

with $T(t)$ in Eq.~\eqref{eqn:accumulate_transmittance_integral} as the accumulated transmittance
along a ray from the near bound $t_n$ to $t$. $\sigma(t)$ and $\boldsymbol{c}(t)$ are the
density and color at the 3D coordinate $\boldsymbol{r}(t)$, respectively.

\begin{equation}
\begin{aligned}
\label{eqn:rendering_integral_quadratur}
&\qquad\qquad\boldsymbol{\hat{C}}(\boldsymbol{r}) = \sum\limits_{i=1}^N T_{i}(\alpha_i) c_{i}, \text{\:where \:}\\
& T_{i}=\mathrm{exp}(- \sum_{j=1}^{i-1} \sigma_{i} \delta_{i}) \text{\:\:and \:\:} \alpha_i = 1 - \mathrm{exp}(- \sigma_{i} \delta_{i}).
\end{aligned}
\end{equation}

The continuous rendering functions \eqref{eqn:rendering_integral} and
\eqref{eqn:accumulate_transmittance_integral} are approximated with numerical quadrature in Eq.
\eqref{eqn:rendering_integral_quadratur}. To make the MLP more generalizable and
prevent overfitting to one set of discrete points, samples are generated randomly between $t_n$
and $t$. This ensures a smoother, continuous representation despite it being evaluated at a
fixed set of discrete points at each training step.

%
The function is optimized given some distance between two sampling points,
$\delta_{i}=t_{i+1}-t_i$, over $\alpha$, denoting the value
used for alpha compositing. In addition to $\alpha$, the equation for $\boldsymbol{\hat{C}}$ is differentiable with
respect to the outputs $(\boldsymbol{c}, \sigma)$, therefore it can be optimized with respect to
a ground truth pixel color $\boldsymbol{C}$. The rendering loss can be expressed as

\begin{equation}
\label{eq:nerf_loss}
\mathcal{L} = \sum_{\boldsymbol{r}\in\mathcal{R}}\left[\left|\left| \hat{C}(\boldsymbol{r}) - C(\boldsymbol{r}) \right|\right|_2^2 \right].
\end{equation}

